Accidental Light Probes

Recovering lighting in a scene from a single image is a fundamental problem in computer vision. While a mirror ball light probe can capture omnidirectional lighting, light probes are generally unavailable in everyday images. In this work, we study recovering lighting from accidental light probes (ALPs) -- common, shiny objects like Coke cans, which often accidentally appear in daily scenes. We propose a physically-based approach to model ALPs and estimate lighting from their appearances in single images. The main idea is to model the appearance of ALPs by photogrammetrically principled shading and to invert this process via differentiable rendering to recover incidental illumination. We demonstrate that we can put an ALP into a scene to allow high-fidelity lighting estimation. Our model can also recover lighting for existing images that happen to contain an ALP.

==> fig_tex/bill_with_emap.tex <==



\begin{figure}[h]
\begin{small}\vspace{-0.1in}
\begin{minipage}{1\linewidth}
\setlength{\columnsep}{4pt}%
\setlength{\intextsep}{0pt}%
\begin{wrapfigure}{l}{55mm}
    \includegraphics[width=\linewidth,clip,keepaspectratio]{figures/bill_with_emap.pdf}
  \end{wrapfigure}\par
Figure R3. For an in-the-wild image, we insert a diet Coke can by estimated lighting. The resolution of the diet Pepsi is about $140\times 70$. Upper-left insets are estimated environment maps. 
\end{minipage}
\end{small}
\vspace{-0.15in}
\end{figure}








==> fig_tex/casual_setup.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.6\linewidth]{figures/casual_setup.pdf}
\vspace{-0.1in}
\caption{Casual multi-view images for ALP reconstruction. We compare our ALP reconstruction pipeline to \cite{munkberg2022extracting, hasselgren2022shape} using casually captured multi-view images of a diet coke can in contrast to using our lightbox setup that is referenced in the main paper. }
\label{fig:supp_casual}
\end{figure*}

==> fig_tex/diff_scales.tex <==
\begin{figure}[h]
\centering\vspace{-0.05in}
\includegraphics[width=1\linewidth]{figures/diff_scales.pdf}
\vspace{-0.3in}
\captionof{figure}{Estimated lighting under different object scales. Insets are input images. Our results are consistent and better.}
\vspace{-0.1in}
\label{fig:diff_scales}
\end{figure}


==> fig_tex/extreme_pose.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=.6\linewidth]{figures/extreme_poses.pdf}
\captionof{figure}{Estimated poses under varying pose conditions. The second row shows re-renderings (which have black backgrounds) overlayed on top of input images. They match accurately.}
\label{fig:extreme_poses}
\vspace{-0.1in}
\end{figure}


==> fig_tex/new_objects.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.6\linewidth]{figures/new_objects.pdf}
\captionof{figure}{ALPs of different shapes (a golden Bird Statue vs.\ golden Ornament 1) and reflectance (Ornaments: 1 and 2 are different in roughness; 1 and 3 are different in albedo).}
\label{fig:new_objects}
\end{figure}


==> fig_tex/supp_indoor.tex <==

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{figures/relight_indoor_supp.pdf}
\vspace{-0.2in}
\caption{Additional qualitative results for indoor scenes. We compare our approach to StyleLight~\cite{wang2022stylelight}, Deep Parametric~\cite{gardner2019deep} and Garon et al~\cite{garon2019fast} on relighting mirror, shiny and diffuse spheres.}
\label{fig:indoor_supp}
\end{figure*}

==> fig_tex/supp_mat.tex <==
\begin{figure*}[ht!]
\centering
\includegraphics[width=\linewidth]{figures/mat_supp.pdf}
\vspace{-0.3in}
\caption{Qualitative comparison of the materials and geometry of a Diet Coke can using our method and \cite{munkberg2022extracting, hasselgren2022shape} in both setups.}
\label{fig:mat_sup}
\end{figure*}

==> fig_tex/supp_outdoor.tex <==

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{figures/relight_outdoor_supp.pdf}
\vspace{-0.3in}
\caption{Additional qualitative results for outdoor scenes, comparing to StyleLight~\cite{wang2022stylelight}, Deep Parametric~\cite{gardner2019deep} and Garon et al~\cite{garon2019fast}.}
\label{fig:outdoor_supp}
\end{figure*}

==> tbl_tex/supp_abl_casual.tex <==


\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{l|ccc|ccc}
        \toprule
        & \multicolumn{3}{c|}{Casual multi-view} & \multicolumn{3}{c}{Lightbox setup} \\
        Method  &  Mirror & Shiny & Diffuse  & Mirror & Shiny & Diffuse \\
        \midrule
        Nvdiffrec~\cite{munkberg2022extracting} & 12.23 & 10.99 & 9.14 & 6.99 & 5.06 & 3.59 \\
        Nvdiffrecmc~\cite{hasselgren2022shape} & 8.76 & 7.37 & \textbf{4.71} &  6.55 & 4.60 & 3.84 \\
        ALP (Ours) & \textbf{6.49} & \textbf{5.48} & 4.89  & \textbf{5.46} & \textbf{3.67} & \textbf{2.80} \\
        \bottomrule
    \end{tabular}
    \caption{Evaluation on our ALP model acquisition for a diet coke can under two different capture settings: casual multi-view images and our lightbox setup. We use the same lighting estimation approach for compared methods and report average angular error across all test scenes.}
    \label{tbl:supp_abl_casual}
\end{table*}

